Sizing Strategies for Algorithmic Trading in Volatile Markets: A Study of Backtesting and Risk Mitigation Analysis

Backtest is a way of financial risk evaluation which helps to analyze how our trading algorithm would work in markets with past time frame. The high volatility situation has always been a critical situation which creates challenges for algorithmic traders. The paper investigates different models of sizing in financial trading and backtest to high volatility situations to understand how sizing models can lower the models of VaR during crisis events. Hence it tries to show that how crisis events with high volatility can be controlled using short and long positional size. The paper also investigates stocks with AR, ARIMA, LSTM, GARCH with ETF data.

==> chapters/references.tex <==
\begin{thebibliography}{99}

\bibitem{criterion35kelly}
  Kelly, JL (1956).
  "A New Interpretation of Information Rate."
  \textit{Bell System Technical Journal},
  35(4), 917--926.

\bibitem{latane1959criteria}
  Latane, Henry Allen (1959).
  "Criteria for choice among risky ventures."
  \textit{Journal of Political Economy},
  67(2), 144--155.
  The University of Chicago Press.

\bibitem{thorp1969optimal}
  Thorp, Edward O (1969).
  "Optimal gambling systems for favorable games."
  \textit{Revue de l'Institut International de Statistique},
  273--293.
  JSTOR.

\bibitem{thorp1975portfolio}
  Thorp, Edward O (1975).
  "Portfolio choice and the Kelly criterion."
  In: \textit{Stochastic optimization models in finance}, 599--619.
  Elsevier.

\bibitem{thorp1980kelly}
  Thorp, Edward O (1980).
  "The Kelly money management system."
  \textit{Gambling Times}, 91--92.

\bibitem{maclean2011kelly}
  MacLean, Leonard C, Thorp, Edward O, \& Ziemba, William T (2011).
  "The Kelly capital growth investment criterion: Theory and practice."
  Volume 3.
  World Scientific.

\bibitem{browne1999risk}
  Browne, Sid (1999).
  "The risk and rewards of minimizing shortfall probability."
  \textit{The Journal of Portfolio Management},
  25(4), 76--85.
  Institutional Investor Journals Umbrella.

\bibitem{hakansson1995capital}
  Hakansson, Nils H, Ziemba, William T, \& others (1995).
  "Capital growth theory."
  In: \textit{Handbooks in operations research and management science}, 9, 65--86.
  Elsevier Amsterdam.

\bibitem{maclean2011time}
  Maclean, Leonard C, Ziemba, William T, \& Li, Yuming (2011).
  "Time to wealth goals in capital accumulation."
  In: \textit{THE KELLY CAPITAL GROWTH INVESTMENT CRITERION: THEORY and PRACTICE}, 259--271.
  World Scientific.

\bibitem{wilcox2003harry}
  Wilcox, Jarrod W (2003).
  "Harry Markowitz and the discretionary wealth hypothesis."
  \textit{The Journal of Portfolio Management},
  29(3), 58--65.
  Institutional Investor Journals Umbrella.

\bibitem{pilar9comprehensive}
  Abad Pilar, Benito Sonia, \& Lopez Carmen.
  "A Comprehensive Review of Value at Risk Methodologies."
  \textit{The Spanish Review of Financial Economics}.


\bibitem{barone1999var}
  Barone-Adesi, Giovanni, Giannopoulos, Kostas, \& Vosper, Les (1999).
  "VaR without correlations for portfolios of derivative securities."
  \textit{Journal of Futures Markets},
  19(5), 583--602.
  Wiley Online Library.

\bibitem{sommacampagna2002estimating}
  Sommacampagna, Cristina (2002).
  "Estimating Value-at-Risk with the Kalman Filter."
  \textit{RIVISTA DI POLITICA ECONOMICA},
  92(11/12), 137--162.

\bibitem{doric2016return}
  Dorić, D (2016).
  "Return distribution and value at risk estimation for BELEX15."
  \textit{Yugoslav Journal of Operations Research},
  21(1).

\bibitem{box1970distribution}
  Box, George EP, \& Pierce, David A (1970).
  "Distribution of residual autocorrelations in autoregressive-integrated moving average time series models."
  \textit{Journal of the American statistical Association},
  65(332), 1509--1526.
  Taylor \& Francis Group.

\bibitem{ljung1978measure}
  Ljung, Greta M, \& Box, George EP (1978).
  "On a measure of lack of fit in time series models."
  \textit{Biometrika},
  65(2), 297--303.
  Oxford University Press.

\bibitem{pelletier2016geometric}
  Pelletier, Denis, \& Wei, Wei (2016).
  "The geometric-VaR backtesting method."
  \textit{Journal of financial econometrics},
  14(4), 725--745.
  Oxford University Press.

\bibitem{pajhede2015backtesting}
  Pajhede, Thor (2015).
  "Backtesting Value-at-Risk: A Generalized Markov Framework."
  \textit{Univ. of Copenhagen Dept. of Economics Discussion Paper},
  (15-18).

\bibitem{hamilton1994time}
  Hamilton, James D (1994).
  "Time series analysis."
  Volume 2.
  Princeton New Jersey.

\bibitem{harvey1990forecasting}
  Harvey, Andrew C (1990).
  "Forecasting, structural time series models and the Kalman filter."
  Cambridge university press.

\bibitem{wells1994variable}
  Wells, Curt (1994).
  "Variable betas on the Stockholm exchange 1971-1989."
  \textit{Applied Financial Economics},
  4(1), 75--92.
  Taylor \& Francis.

\bibitem{massey1951kolmogorov}
  Massey Jr, Frank J (1951).
  "The Kolmogorov-Smirnov test for goodness of fit."
  \textit{Journal of the American statistical Association},
  46(253), 68--78.
  Taylor \& Francis.

\bibitem{gumparthi2017relative}
  Gumparthi, Srinivas (2017).
  "Relative strength index for developing effective trading strategies in constructing optimal portfolio."
  \textit{International Journal of Applied Engineering Research},
  12(19), 8926--8936.

\bibitem{bollinger2002bollinger}
  Bollinger, John (2002).
  "Bollinger on Bollinger bands."
  McGraw Hill Professional.

\bibitem{johnston1999some}
  Johnston, FR, Boyland, JE, Meadows, M, \& Shale, E (1999).
  "Some properties of a simple moving average when applied to forecasting a time series."
  \textit{Journal of the Operational Research Society},
  50(12), 1267--1271.
  Taylor \& Francis.

\bibitem{chande1994new}
  Chande, Tushar S, \& Kroll, Stanley (1994).
  "The new technical trader: boost your profit by plugging into the latest indicators."
  Volume 44.
  John Wiley \& Sons Incorporated.

\bibitem{batten1996technical}
  Batten, Jonathan, \& Ellis, Craig (1996).
  "Technical trading system performance in the Australian share market: Some empirical evidence."
  \textit{Asia Pacific Journal of Management},
  13(1), 87--99.
  Springer.

\bibitem{headley2002big}
  Headley, Price (2002).
  "Big trends in trading: Strategies to master major market moves."
  Volume 145.
  John Wiley \& Sons.

\bibitem{burgers1999nino}
  Burgers, Gerrit (1999).
  "The El Nino stochastic oscillator."
  \textit{Climate Dynamics},
  15(7), 521--531.
  Springer.

\bibitem{thomsett2010cmf}
  Thomsett, Michael C (2010).
  "CMF--Chaikin Money Flow: Changes Anticipating Price Reversal."
  FT Press.

\bibitem{wilder1978momentum}
  Wilder Jr, J Welles (1978).
  "A Momentum Oscillator that Can Help You Spot Market Turns."
  \textit{Commodities},
  7, 46--47.

\bibitem{evens1999keltner}
  Evens, Stuart (1999).
  "Keltner Channels."
  \textit{TECHNICAL ANALYSIS OF STOCKS AND COMMODITIES-MAGAZINE EDITION-},
  17, 45--48.
  TECHNICAL ANALYSIS, INC.

\bibitem{tharavanij2017profitability}
  Tharavanij, Piyapas, Siraprapasiri, Vasan, \& Rajchamaha, Kittichai (2017).
  "Profitability of Candlestick Charting Patterns in the Stock Exchange of Thailand (SET)."
  \textit{SAGE Open},
  7(4), 1--18.

\bibitem{elliott2007ichimoku}
  Elliott, Nicole (2007).
  "Ichimoku Charts: An Introduction to Ichimoku Kinko Clouds."
  Harriman House Limited.

\end{thebibliography}


==> core/acknowledgement.tex <==
\section*{Acknowledgement}
Firstly, all praise to the Great Allah for whom my thesis have been completed without any major interruption.\\
Secondly, to my advisor Mahbubul Alam Majumdar sir for his kind support and advice in our work. He helped us whenever we needed help.\\
Thirdly, to Tanjima Nasreen Jenia, who inspired me and reviewed the paper while writing this thesis. 

==> core/approval.tex <==
\section*{Approval}

The thesis titled “Sizing in Financial Trading” submitted by 
\begin{enumerate}
  \item S. M. Masrur Ahmed (16301087)
\end{enumerate}

Of Spring, 2020 has been accepted as satisfactory in partial fulfillment of the requirement for the degree of B.Sc. in Computer Science on March 7, 2020. 

\vspace{0.5cm}
\textbf{Examining Committee:}

\vspace{1cm}

Supervisor:
(Member)
\begin{center}
    \hspace{7cm} \wildcard{\centerline{Mahbubul Alam Majumdar} \\ \centerline{Professor and Dean, School of Data and Sciences}\centerline{BRAC University}} \hspace{1cm} 
\end{center}

Program Coordinator:
(Member)
\begin{center}
    \hspace{7cm} \wildcard{\centerline{Md. Golam Rabiul Alam} \\ \centerline{Associate Professor}\\ \centerline{Department of Computer Science and Engineering}\\ \centerline{BRAC University}} \hspace{1cm} 
\end{center}

Head of Department:
(Chair)
\begin{center}
    \hspace{7cm} \wildcard{\centerline{Mahbubul Alam Majumdar} \\ \centerline{Professor and Dean, School of Data and Sciences} \centerline{BRAC University}} \hspace{1cm} 
\end{center}

\pagebreak

==> core/declaration.tex <==
% Following command is used to created grouped signature line for Four Authors
\newcommand*\wildcard[2][6cm]{\vspace{2cm}\parbox{#1}{\hrulefill\par#2}} 

% A "parbox{}{}" is a box whose contents are created in paragraph mode. 
% "hrulefill{} to chance thickness of underline"

\section*{Declaration}

It is hereby declared that

\begin{enumerate} % begin{enumerate} function to create numbered list
  \item The thesis submitted is my/our own original work while completing degree at BRAC University.
  \item The thesis does not contain material previously published or written by a third party, except where this is appropriately cited through full and accurate referencing.
  \item The thesis does not contain material which has been accepted, or submitted, for any other degree or diploma at a university or other institution.
  \item We have acknowledged all main sources of help.
\end{enumerate}

\vspace{1cm}
\textbf{Student’s Full Name \& Signature:} % Testbf{} for Bold

\begingroup

    \begin{center}
        \wildcard{\centerline{S. M. Masrur Ahmed} \\ 
        \centerline{16301087}} 
    \end{center}

\endgroup


\pagebreak







==> core/dedication.tex <==
\section*{Dedication}
To my parents, You guys forever have forever been an inspiration to me. Your adore and support were the keys for me to run for my aim. 
\pagebreak
